Quantitatively Nonblocking Supervisory Control of Discrete-Event Systems

In this paper, we propose two new nonblocking properties of automata as quantitative measures of maximal distances to marker states. The first property, called {\em quantitative nonblockingness}, captures the practical requirement that at least one of the marker states (representing e.g. task completion) be reachable within a prescribed number of steps from any non-marker state and following any trajectory of the system. The second property, called {\em heterogeneously quantitative nonblockingness}, distinguishes individual marker states and requires that each marker state be reached within a given bounded number of steps from any other state and following any trajectory of the system. Accordingly, we formulate two new problems of quantitatively nonblocking supervisory control and heterogeneously quantitatively nonblocking supervisory control, and characterize their solvabilities in terms of new concepts of quantitative language completability and heterogeneously quantitative language completability, respectively. It is proved that there exists the unique supremal (heterogeneously) quantitatively completable sublanguage of a given language, and we develop effective algorithms to compute the supremal sublanguages. Finally, combining with the algorithm of computing the supremal controllable sublanguage, we design algorithms to compute the maximally permissive solutions to the formulated (heterogeneously) quantitatively nonblocking supervisory control problems.

==> SubSect_SupComplet-Gen.tex <==

{\it 4.2.1. Generator-Based Approach}

Let $K$ be represented by a (nonblocking) generator ${\bf K} = ({X, \Sigma, \xi, x_{0}, X_{m}})$, i.e. $L_m({\bf K}) = K$ and $L({\bf K}) = \overline{K}$.
The intuition is that we find for each state of ${\bf K}$ the quantitatively completable strings, and remove
other non-quantitatively completable strings from the transition graph. The detailed steps are described in Algorithm~\ref{algm:supnc}. In the algorithm,
we employ a last-in-first-out stack $ST$ to store the states to be processed (a first-in-first-out queue can also be used instead to perform a different order of search), and for a set $Z$ a flag $F:Z \rightarrow \{true, false\}$ to
indicate whether or not an element of $Z$ has been visited: $F(z) = true$ represents that $z \in Z$ has been visited.

%\begin{algm}[Algorithm of Computing $\sup\mathcal{QC}(K, N)$] \label{algm:supnc}
%\begin{figure}[!t]
\begin{algorithm}[htbp]
\caption{: Algorithm of Computing $\sup\mathcal{QC}(K, \{P_i\}, \{N_i\})$}
\label{algm:supnc}
%~\\
%\noindent\rule{\columnwidth}{1pt}

\noindent {\bf Input}: Generator ${\bf K} = ({X, \Sigma, \xi, x_{0}, X_{m}})$ representing $K$, a marker state set $P_i \subseteq Q_m(K)$, and a positive integer $N_i$.\\
\noindent {\bf Output}: Generator ${\bf K}_i'= (X_i', \Sigma, \xi_i', x'_{i,0}, X_{i,m}')$.
\\
\\
\noindent {\bf Step 1.} Let ${\bf G}_i = (Q,\Sigma, \delta, q_0, P_i)$, and compute the product
generator ${\bf GK}_i$ of ${\bf G}_i$ and $\bf K$; write
${\bf GK}_i = (X_i, \Sigma, \xi_i, x_{i,0}, X_{i,m})$, where $X_i \subseteq (Q\times X)$ and $X_{i,m} \subseteq P_i \times X_m$.
\\
\\
\noindent {\bf Step 2.} Let
\[X_i' := \{(x_i,d)|x_i\in X_i, d \in \{0,...,N_i-1\}\},\]
$\xi_i' = \emptyset$, $x_{i,0}' = (x_{i,0},0)$, and $X_{i,m}' := \{(x_i,0)|x_i\in X_{i,m}\}$. Initially set $F((x_i,d)) = false$ for each state $x_i \in X_i$ and each $d \in \{0,...,N_i-1\}$.
Then push the initial state $x_{i,0}'=(x_{i,0},0)$ into stack $ST$, and set $F((x_{i,0},0)) = true$.
\\
\\
\noindent {\bf Step 3.} If stack $ST$ is empty, trim\footnotemark the generator ${\bf K}_i' = (X_i', \Sigma, \xi_i', x'_{i,0}, X_{i,m}')$, and go to Step 6.
Otherwise, pop out the top element $(x_{i,j}, d)$ of stack $ST$. If $x_{i,j} \in X_{i,m}$, go to Step 4; otherwise, go to Step 5.
\\
\\
\noindent {\bf Step 4.} For each event $\sigma \in \Sigma$ defined at state $x_{i,j}$ (i.e. $\xi(x_{i,j},\sigma)!$), let $x_{i,k} := \xi(x_{i,j},\sigma)$ and do the following two steps 4.1 and 4.2;
then go to Step 3 with updated stack $ST$.\\
\\
\indent~~ {\bf Step 4.1} Add transition $((x_{i,j},0),\sigma,(x_{i,k},0))$ to $\xi'$, i.e.
\[\xi' := \xi' \cup \{((x_{i,j},0),\sigma, (x_{i,k},0))\}.\]
\indent~~ {\bf Step 4.2} If $F((x_{i,k},0)) = false$, push $(x_{i,k},0)$ into stack $ST$ and set $F((x_{i,k},0)) = true$.
\\
\\
\noindent {\bf Step 5.} For each event $\sigma \in \Sigma$ defined at state $x_{i,j}$ (i.e. $\xi(x_{i,j},\sigma)!$), let $x_{i,k} := \xi(x_{i,j},\sigma)$ and do the following three steps 5.1--5.3;
then go to Step 3 with updated stack $ST$.
\\
\indent~~ {\bf Step 5.1} If $x_{i,k} \in X_{i,m}$, set $d' = 0$; if $x_{i,k} \notin X_{i,m}$, set $d' = d + 1$.
\\
\indent~~ {\bf Step 5.2} If $d' = N$, go to Step 4.1 with the next event $\sigma$ defined at $x_{i,j}$; if no more events are defined at $x_{i,j}$, go to Step 4.4.
Otherwise, add a new transition $((x_{i,j},d),\sigma, (x_{i,k},d'))$ to $\xi'$, i.e.
\[\xi' := \xi' \cup \{((x_{i,j},d),\sigma, (x_{i,k},d'))\}\]
\indent~~ {\bf Step 5.3} If $F((x_{i,k},d')) = false$, push $(x_{i,k},d')$ into stack $ST$ and set $F((x_{i,k},d')) = true$.
\\
\\
\noindent {\bf Step 6.} For each state $x_i' \in X_i' \subseteq X_i\times\{0,...,N_{i-1}\} \subseteq Q\times X \times \{0,...,N_{i-1}\}$, let $x \in X$
be the state of $\bf K$ corresponding to $x_i'$. If $x_i' \notin X_{i,m}'$ but $x \in X_m$, add $x_i'$ to the marker state set $X_{i,m}'$.
%\noindent\rule{\columnwidth}{1pt}
\end{algorithm}
%\end{figure}
\footnotetext{`Trimmed' means all non-reachable and non-coreachable states (if they exist) are removed \cite{Elienberg:1974, Wonham16a}.
The generator ${\bf K}'$ generator may be not already trim, and to get a nonblocking generator, this step is a required computation step.  }

In Step 4.2 above, note that the condition $d' = N$ means that the $N$-step downstream transitions that have never
reached a marker state will be removed, therefore guaranteeing that from an arbitrary state, at most $N$-step transitions
are needed to reach a marker state.
Also note that Step 6 is necessary, because in Step 1, the strings in $K$ but don't visit any marker state in
$P_i$ are excluded, but those strings should be included in the marked behavior $L_m({\bf K}_i')$, and as will be
shown in the Theorem 1, this step will not break the quantitative completability of ${\bf K}_i'$ obtained by
Step 3.
% {\color{red}Also note that $\bf G$ is not an input of Algorithm~\ref{algm:supnc}. The reason is as follows.
%Since $K \subseteq L_m({\bf G})$, each string $s \in K$ corresponds to a marker state in $\bf G$, and the property of quantitative completability requires that `one of' the marker states
%of $\bf G$ must be reached in $N$-steps, and thus it is unnecessary to distinguish which marker state the string $s$ corresponds to. }

\begin{example} [Continuing Example 1]
Inputting $L_m({\bf SUP})$  and $N = 3$, Algorithm 1 outputs a new generator ${\bf SUP}'$, as displayed in Fig.~\ref{fig:SUP'}. From the figure, we see that non-marker states 0, 3, 4, 5, 6, 7, 8, 9 are guaranteed to reach the marker states 1 or 2 in at most 3 steps.
By contrast in ${\bf SUP}$ (displayed in Fig.~\ref{fig:GSUP}), the strings $(19.17)^{N}.24$ with $N \geq 3$ will also lead unmarked state 3 to the marker state 2; however, their lengths are greater than 3. Thus, in fact those strings are removed from ${\bf SUP}$ by Algorithm~1. \hfill $\diamond$
%\setlength{\floatsep}{1pt plus 2pt minus 2pt}
\begin{figure}[!htbp]
\centering
\begin{minipage}{0.5\textwidth}
\centering
 \includegraphics[scale = 0.34]{Figures/SUPprim.pdf}
\end{minipage}
%\vspace{-0.1cm}

\begin{minipage}{0.5\textwidth}
\centering
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{|c|c||c|c|}
  \hline
   $x' \in X'$ &  $(x,d) \in X\times N$& $x' \in X'$ &  $(x,d) \in X\times N$ \\
   \hline
  0 & (0,0) & 5 & (4,1)\\
  \hline
  1 & (1,0)& 6 & (3,1) \\
  \hline
  2 & (2,0) & 7 & (3,2)\\
  \hline
  3 & (3,0) & 8 & (5,1) \\
  \hline
  4 & (4,0) & 9 & (0,2)\\
  \hline
\end{tabular}
}
\end{minipage}
\caption{Transition graph of ${\bf SUP}'$ and state correspondences between ${\bf SUP}'$ and ${\bf SUP}$ } \label{fig:SUP'}
\vspace{-0.2cm}
\end{figure}
\end{example}
%\begin{figure}[ht]
%\centering
%    \includegraphics[scale = 0.15]{Figures/KE.pdf}
%\caption{Transition graphs of ${\bf SUPE}$  } \label{fig:SF_Layout}
%\end{figure}

The correctness of Algorithm 1 is confirmed by the following theorem.

\begin{thm} \label{thm:algmcompute}
Given a language $K \subseteq L_m({\bf G})$, a marker state set $P_i \subseteq Q_m(K)$ and a positive integer $N_i$, and let ${\bf K}_i'$ be the generator returned by Algorithm~1. Then
$L_m({\bf K}_i') = \sup\mathcal{QC}(K, \{P_i\}, \{N_i\})$.
\end{thm}

%Due to space limit, we refer the reader to  \cite{ZhangWangCaiArxiv:2021} for a proof of Theorem~\ref{thm:algmcompute}.

{\it Proof:}
First, we prove that $L_m({\bf K}_i') \in \mathcal{QC}(K, \{P_i\}, \{N_i\})$.
We start by showing that $L_m({\bf K}_i') \subseteq K$. The reasons are as follows. (i) In Steps 4 and 5, all the transitions
added to ${\bf K}_i'$ correspond to those existing in ${\bf K}$, so $L({\bf K}_i') \subseteq L({\bf K}) = \overline{K}$.
(ii) Since marker states in ${\bf K}_i'$ are on the one hand copied from ${\bf K}$ by $X_{i,m}' := \{(x_i,0)|x_i\in X_{i,m}\}$ in Step 2
and on the other hand added from $X_m$ in Step 6, $L_m({\bf K}_i') \subseteq L({\bf K}_i') \cap L_m({\bf K}) \subseteq K$.

Next we show that $L_m({\bf K}_i')$ is quantitatively completable wrt. $\{(P_i, N_i)\}$. Before Step 6, it is guaranteed by  $d' = N_i$ in Step 5.2 that if a string is longer than $N$ and has never reached a marker
state, then it will not be added to $L({\bf K}_i')$. Thus, those strings $s$ added to $L({\bf K}_i')$ must satisfy
that for every $t \in M_{L_m({\bf K}_i')}(s)$, there holds $|t| \leq N_i$. After Step 6, since we only add (not remove) marker states to ${\bf K}_i'$,
for each $t \in M_{L_m({\bf K}_i')}(s)$, only its prefixes $t' \leq t$ are still kept in $M_{L_m({\bf K}_i')}(s)$ ; thus
for every $t' \in M_{L_m({\bf K}_i')}(s)$, we have $|t'| \leq |t| \leq N_i$.  Hence, $L_m({\bf K}_i')$ is quantitatively
completable wrt. $\{(P_i, N_i)\}$.  This establishes $L_m({\bf K}_i') \in \mathcal{QC}(K, \{P_i\}, \{N_i\})$.

It remains to show that $L_m({\bf K}_i')$ is the largest element in $\mathcal{QC}(K, \{P_i\}, \{N_i\})$.
Let $M \subseteq K$ be another element in $\mathcal{QC}(K, \{P_i\}, \{N_i\})$. It will be shown that  $M \subseteq L_m({\bf K}_i')$. For this, we first prove that $\overline {M} \subseteq L({\bf K}_i')$ by induction on the length of a string $s \in \overline{M}$.

{\bf Base case:} Let $s = \epsilon \in \overline{M}$. Then $\epsilon \in \overline{K}$ and the initial state $x_{i,0}$ exists in {\bf K}. It follows from Step~1 that $x'_{i,0} = (x_{i,0},0)$ is designated to be the initial state of ${\bf K}_i'$, and hence $\epsilon \in L({\bf K}')$.

{\bf Inductive case:} Let $s \in \overline{M}$, $s \in L({\bf K}_i')$, $\sigma \in \Sigma$, and suppose that $s\sigma \in \overline{M}$; we will show that $s\sigma \in L({\bf K}_i')$ as well.
Since $M \in \mathcal{QC}(K, \{P_i\}, \{N_i\})$, we have (i) $M \subseteq K$ and (ii) $M$ is quantitatively completable wrt. $\{(P_i, N_i)\}$.
It follows from (i) and $L({\bf K}) \cap L({\bf G}) = L({\bf K})$ that $s \in L({\bf K}) \cap L({\bf G})$, i.e.
$\xi_i(x_{i,0}, s)!$. By the same reason, $\xi_i(x_{i,0},s\sigma)!$. Letting $x_i = \xi_i(x_{i,0}, s)$, we derive $\xi_i(x_i,\sigma)!$. Since $s \in L({\bf K}_i')$, $\xi_i'((x_{i,0},0),s)!$.
According to the definition of $\xi_i'$, there must exist $d \in \{0,...,N-1\}$ such that $(x_i,d) = \xi_i'((x_{i,0},0),s)$.
We have already known that $\xi_i(x_i,\sigma)!$. If $x_i \in X_{i,m}$, according to Step 4, $\xi_i'((x_i,d),\sigma)$ is defined where $d =0$.
If $x_i \notin X_{i,m}$, according to Step 5.1, if $\xi_i(x_i,\sigma) \in X_{i,m}$, $d' = 0$; otherwise $d' = d + 1$.
For the former case, according to Step 5.2, $\xi_i'((x_i,d),\sigma)$ is defined with $d' = 0$. For the latter case,
it must hold that $d' \leq N_i-1$ because $\xi_i(x_i,\sigma) \notin X_{i,m}$ and $M$ is quantitatively completable (otherwise
there exists a string $s' \in \overline{M}$ and $t \in M_M(s)$ such that $|t| = N_i +1$). According to Step 5.2, in this
case  $\xi_i'((x_i,d),\sigma)$ is also defined. Hence, we conclude that $s\sigma \in L({\bf K}_i')$.

Therefore, by the above induction, $\overline {M} \subseteq L({\bf K}_i')$ is established.
Moreover we prove that $L({\bf K}_i') \cap L_m({\bf K}) \subseteq L_m({\bf K}_i')$.
Let $s \in L({\bf K}_i')$ and $s \in L_m({\bf K})$;
then we have $\xi_i'((x_{i,0},0),s)!$ and $\xi(x_0,s) \in X_m$. According to whether or not $\delta(q_0,s) \in P_i$,
we have (i) $\xi_i(x_0,s) \in X_{i,m}$ and (ii) $\xi(x_0,s) \in X_m$ but $\xi_i(x_0,s) \notin X_{i,m}$
In case (i), according to Steps 2 and 5.1, when $\xi(x_{i,0},s) \in X_{i,m}$, $d' = 0$.
Since $X_{i,m}' = \{(x_i,0)|x_i\in X_{i,m}\}$, we have $\xi_i'((x_{i,0},0),s) \in X_{i,m}'$.
In case (ii), since $\xi(x_0,s) \in X_m$, $\xi_i'((x_{i,0},0),s)$ is added to $X_{i,m}'$ by Step 6. Hence, we conclude that $s \in L_m({\bf K}_i')$.
Finally,
\begin{align*}
M &\subseteq \overline{M} \cap L_m({\bf K})\\
    & \subseteq L({\bf K}_i') \cap L_m({\bf K}) \\
    & \subseteq L_m({\bf K}_i').
\end{align*}
The proof is now complete. \hfill $\blacksquare$


The above theorem confirms that Algorithm 1 computes the supremal quantitatively completable sublanguage $\sup\mathcal{QC}(K, N)$.
According to Steps 3 and 4, the time complexity of Algorithm 1 is $O(|X|\cdot|\Sigma|\cdot N)$ where $|X|$ is the state number of automaton
$\bf K$, because
${\bf K}$ has at most $|X| \cdot |\Sigma|$ transitions and each transition is visited at most $N-1$ times.
Namely, this algorithm is pseudo-polynomial in the states number $|X|$ of $\bf K$. Compared with the language-based algorithm of computing
$\sup\mathcal{QC}(K, N)$ in the previous subsection which has complexity $O(|X|^3 \times |\Sigma|\times N^2)$, this generator-based
algorithm is more efficient.



==> Subsect_StrongCompletControl.tex <==
%\subsection{Maximally Permissive Strongly $N$-Step Nonblocking Supervisory Control}

In this subsection, we present our solution to the  HQNSCP.
Consider a DES plant modeled by a generator ${\bf G}$ as in (\ref{eq:plant}) with $\Sigma = \Sigma_c \dot\cup \Sigma_{uc}$, and a specification language $E \subseteq \Sigma^*$. Let $K := E \cap L_m({\bf G})$, $Q_m(K)$ as defined in ~(\ref{eq:QmKL}), and $N_i$ a positive integer for each $q_{m,i} \in Q_m(K)$.

Whether or not $K$ is controllable and heterogeneously quantitatively completable, let $\mathcal{CHQC}(K, Q_m(K), \{N_i| i \in \mathcal{I}\})$ be the set of sublanguages of $K$ that are both controllable and heterogeneously quantitatively completable wrt. $\{(q_{m,i}, N_i)|i \in \mathcal{I}\}$, i.e.
\begin{align*}
\mathcal{CHQC}&(K, Q_m(K), \{N_i| i \in \mathcal{I}\}) :=\{K' \subseteq K \mid K'~ \text{is both}\\
& \text{controllable and heterogeneously quantitatively}\notag\\
&\text{completable wrt. $\{(q_{m,i}, N_i)|i \in \mathcal{I}\}$}\}.
\end{align*}
Since the empty language $\emptyset$ is trivially controllable and heterogeneously quantitatively completable, the set $\mathcal{CHQC}(K, T, \mathcal{N})$ is nonempty. Moreover, since both controllability and heterogeneously  quantitative completability are closed under arbitrary set unions, $\mathcal{CHQC}(K, T, \mathcal{N})$ contains a unique supremal element given by
\begin{align*}
\sup\mathcal{CHQC}(K,Q_m&(K), \{N_i| i \in \mathcal{I}\}) :=\bigcup\{K'\subseteq K \mid \\
&K' \in \mathcal{CHQC}(K,Q_m(K), \{N_i| i \in \mathcal{I}\}) \}.
\end{align*}

Our main result in this subsection is the following.

\begin{thm} \label{thm:chqc}
Suppose that $\sup\mathcal{CHQC}(K, Q_m(K), \{N_i|$ \\$ i \in \mathcal{I}\}) \neq \emptyset$.
Then the supervisory control $V_{hsup}$ such that $L_m(V_{hsup}/{\bf G})=\sup\mathcal{CHQC}(K, Q_m(K), \{N_i| i \in \mathcal{I}\}) \subseteq K$ is the solution to the HQNSCP.
\end{thm}

%For the proof of Theorem~\ref{thm:chqc}, see \cite{ZhangWangCaiArxiv:2021}.
%{\it Proof:}
%Let $\sup\mathcal{CHQC}(K, Q_m(K), \{N_i| i \in \mathcal{I}\})$ be nonempty. According to Theorem~\ref{thm:snsct}, since $\sup\mathcal{CHQC}(K, Q_m(K), $ $ \{N_i| i \in \mathcal{I}\})$ is controllable and heterogeneous quantitative completable, there exists a heterogeneous quantitative nonblocking supervisory control $V_{hsup}$ such that $L_m(V_{hsup}/{\bf G})=\sup\mathcal{CHQC}(K, Q_m(K), \{N_i| i \in \mathcal{I}\}) \subseteq K$. Hence the safety and heterogeneous quantitative nonblockingness requirements of the HQNSCP are satisfied. Further, since $\sup\mathcal{CHQC}(K, Q_m(K), \{N_i| i \in \mathcal{I}\})$ is the supremal element in $\mathcal{CHQC}(K, Q_m(K), \{N_i| i \in \mathcal{I}\})$, the maximal permissiveness requirement of the HQNSCP is also satisfied. Therefore, $V_{hsup}$ that synthesizes $\sup\mathcal{CHQC}(K, Q_m(K), \{N_i| i \in \mathcal{I}\})$ is the solution to the HQNSCP. \hfill $\blacksquare$


We proceed to design an algorithm to compute this solution $\sup\mathcal{CHQC}(K, Q_m(K), \{N_i| i \in \mathcal{I}\})$. The algorithm
consists of the iterative computation of the supremal heterogeneously quantitatively completable sublanguage and the supremal
controllable sublanguage.

\begin{algorithm}[h]
\caption{: Algorithm of Computing $\sup\mathcal{CHQC}(K, $ $Q_m(K), \{N_i| i \in \mathcal{I}\})$}
\label{algm:supcsnc}

\noindent {\bf Input}: Plant generator ${\bf G} = (Q, \Sigma, \delta, q_0, Q_m)$, specification language $E \subseteq \Sigma^*$, ${Q_m(E \cap L_m({\bf G}))} = \{q_{m,i}|i \in \mathcal{I}\}$
and $\{N_i| i \in \mathcal{I}\}$.\\
\noindent {\bf Output}: Generator ${{\bf HQSUP}} = (X, \Sigma, \delta, x_0, X_m)$.
\\

\noindent {\bf Step 1.} Let $K := E \cap L_m({\bf G})$ (thus $Q_m(K) = Q_m(E \cap L_m({\bf G}))$). Construct a nonblocking generator ${\bf K}_0$ such that $L_m({\bf K}_0) = K$.

\noindent {\bf Step 2.} Apply Algorithm~\ref{algm:supsnc} (with inputs ${\bf K}_i$, $Q_m(K) = \{q_{m,i}|i \in \mathcal{I}\}$, and $\{N_i| i \in \mathcal{I}\}$) to compute ${\bf H}_i$ such that $L_m({\bf H}_i) = \sup\mathcal{SQC}(L_m({\bf K}_i), Q_m(K),\{N_i| i \in \mathcal{I}\})$.

\noindent {\bf Step 3.} Apply Algorithm SC (with inputs ${\bf G}$ and $L_m({\bf H}_i)$) to compute ${\bf K}_{i+1}$ such that $L_m({\bf K}_{i+1}) = \sup\mathcal{C}(L_m({\bf H}_i))$.

\noindent {\bf Step 4.} If ${\bf K}_{i+1} ={\bf K}_i$, then output ${{\bf HQSUP}} = {\bf K}_{i+1}$. Otherwise, advance $i$ to $i+1$ and go to {\bf Step~2}.

%\noindent\rule{\columnwidth}{1pt}
\end{algorithm}

The correctness of this algorithm is confirmed by the following theorem.

\begin{thm}\label{thm:supstrongcomctr}
Given a plant generator ${\bf G}$, a specification language $E$, let $K := E \cap L_m({\bf G})$, $Q_m(K) \subseteq Q_m$ a subset of marker states as defined in (\ref{eq:QmKL}), $N_i$ a positive integer for each $q_{m,i} \in Q_m(K)$, and ${{\bf HQSUP}}$ be the generator returned by Algorithm~\ref{algm:supcsnc}. Then $L_m({{\bf HQSUP}}) = \sup\mathcal{CHQC}(K, Q_m(K),\{N_i| i \in \mathcal{I}\})$.
\end{thm}

%The proof of this theorem is similar to that of Theorem~\ref{thm:supcomctr}, with $L_m({\bf H}_i) = \sup\mathcal{QC}(L_m({\bf K}_i), N)$ being replaced
%by $L_m({\bf H}_i) = \sup\mathcal{HQC}(L_m({\bf K}_i),  Q_m(K),\{N_i| i \in \mathcal{I}\})$.
%\end{proof}

Since Algorithm~\ref{algm:supsnc} used in Step~2 has complexity $O\big(|\mathcal{I}|\cdot(|Q|\cdot ||E||_L \cdot |\Sigma|\cdot \prod_{i=1}^{|\mathcal{I}|}{N_i})^2\big)$, Algorithm SC used in Step~3 has complexity $O(|Q|\cdot ||E||_L \cdot |\Sigma|\cdot \prod_{i=1}^{|\mathcal{I}|}{N_i})$, and there can be at most $O(|Q|\cdot ||E||_L \cdot |\Sigma|\cdot \prod_{i=1}^{|\mathcal{I}|}{N_i})$ iterations of Steps~2 and 3, the time complexity of Algorithm~\ref{algm:supcsnc} is $O\big(|\mathcal{I}|\cdot(|Q|\cdot ||E||_L \cdot |\Sigma|\cdot \prod_{i=1}^{|\mathcal{I}|}{N_i})^3\big)$.

\begin{example} [Continuing Example 1]
Consider plant generator ${\bf G}$ and nonblocking supervisor ${\bf SUP}$ displayed in Fig.~\ref{fig:GSUP}).
Input ${\bf G}$, $L_m({\bf SUP})$,  $Q_m(L_m({\bf SUP})) = \{q_{m,1} = 1, q_{m,2} = 2\}$ ($\mathcal{I} = \{1,2\}$) and $\{N_1 = 3, N_2 = 4\}$ to Algorithm~\ref{algm:supcsnc}. In Step~1, ${\bf K}_0 := {\bf SUP}$.
Then in Step~2, Algorithm~\ref{algm:supsnc} generates a generator ${\bf H}_0 = {\bf K_3}$ (displayed in Fig.~\ref{fig:K3}); it is
verified that $L_m({\bf H}_0) = L_m({\bf K}_3)$ is heterogeneously quantitatively completable wrt. $\{(q_{m,1} = 1, N_1 = 3), (q_{m,2} = 2, N_1 = 4)\}$. However, it is not controllable, because uncontrollable event 16 is disabled at states 6 and 11.
Next in Step~3, Algorithm SC generates a generator ${\bf K}_1$ as displayed Fig.~\ref{fig:SNCSUP}.
It is verified that $L_m({\bf K}_1)$ is both controllable and heterogeneously quantitatively completable wrt. $\{(q_{m,1} = 1, N_1 = 3), (q_{m,2} = 2, N_1 = 4)\}$.
This means that in Step~4, although ${\bf K}_1 \neq {\bf K}_0$ and Steps~2 and 3 need to be repeated, no further change will be made. It follows that ${\bf K}_2 = {\bf K}_1$, and Algorithm~3 outputs ${{\bf HQSUP}} = {\bf K}_1$.

\begin{figure}[!t]
\centering
    \includegraphics[scale = 0.34]{Figures/NSSUP.pdf}
\caption{Transition graph of generator ${\bf K}_1$, supervisors ${\bf HQSUP}$ and ${\bf HQSUP1}$  (they have identical transition structure)} \label{fig:SNCSUP}
\vspace{-0.2cm}
\end{figure}

This ${\bf HQSUP}$ may be used as a supervisor for the autonomous vehicle to provide timely services to the customers in zone~1 (three steps) and zone~2 (four steps).
The control logics are as follows: (i) never move to zone~5 when in zone~0; (ii) never move to zone~4 when in zone~1 or zone~3; and (iii)
if the vehicle is in zone 1, it cannot move to zone 0 unless it has just returned back from zone 2. These logics guarantee that
the second requirement (in Section 2.2) on the vehicle can be satisfied; namely, every package sent to a customer in zone 1 (resp.
zone 2) can be delivered by the vehicle to zone 1 (resp.
zone 2) within three steps (resp. four steps), and whenever a customer in
zone 1 (resp. zone 2) calls for package collection, the
vehicle can reach zone 1 (resp. zone 2) within three steps (resp. four steps).

Additionally, we demonstrate that the solution for HQNSCP need not solve QNSCP in the following two cases.
First, consider the case that $N = 3$ which is equal to the minimum of $N_1=3$ and $N_2=4$. It is verified that $L_m({\bf HQSUP})$ is controllable and quantitatively completable wrt. $N = 3$.
Namely, ${\bf HQSUP}$ can act as a supervisor satisfying the safety and quantitative nonblockingness of QNSCP (with $\bf G$, $\bf SUP$ and $N = 3$). However, comparing ${\bf HQSUP}$ with the optimal supervisor $\bf QSUP$ (as displayed in Fig.~\ref{fig:NCSUP}) for QNSUP, we find that there exists strings $(11.29)^N$ in $L_m({\bf QSUP})$, but not in $L_m({\bf HQSUP})$. That is, the repeated visits of zones 0 and 1 is not permitted
for ${\bf HQSUP}$, but is permitted for ${\bf HQSUP}$. Specifically, the vehicle cannot provide timely services to the customers in zone 2 (violating the requirement (i) in Example 1); however, if the visits of zones 1 and 2 are treated the same (as in the requirement (i) in Example 1), the repeated visits of zones 1 and 2 is legal for supplying timely services.
Namely, the maximal permissiveness of QNSCP is not satisfied, which demonstrates that ${\bf HQSUP}$ for HQNSCP is not optimal for solving QNSCP.

Second, consider the case that $N = 1$, and $\{N_1 = 3, N_2 = 1\}$ (i.e. $N$ is again equal to the minimum of $N_1$ and $N_2$).
Applying the algorithm of synthesizing quantitatively nonblocking supervisor with inputs $\bf G$, $L_m({\bf SUP})$ and $N = 1$, we obtain
an optimal supervisor $\bf QSUP'$ (as displayed in Fig.~\ref{fig:QSUP'}) for solving QNSCP. From the figure, we see that $L_m({\bf QSUP}') \neq \emptyset$.
However, applying Algorithm~\ref{algm:supcsnc} with inputs $\bf G$, $L_m({\bf SUP})$, $Q_m({\bf SUP}) = \{q_{m,1} = 1, q_{m,2} = 2\}$ ($\mathcal{I} = \{1,2\}$) and $\{N_1 = 3, N_2 = 1\}$,
we get an empty generator, because marker state 2 cannot be reached in one step from the initial state. This result demonstrates that even when Algorithm~\ref{algm:supcsnc} returns no solution for HQNSCP,
the algorithm of synthesizing quantitatively nonblocking supervisor can find a nonempty optimal supervisor for solving QNSCP.
 ~\hfill $\diamond$

\begin{figure}[!t]
\centering
    \includegraphics[scale = 0.34]{Figures/QSUPprim.pdf}
\caption{Transition graph of $\bf QSUP'$ } \label{fig:QSUP'}
\vspace{-0.2cm}
\end{figure}
\end{example}







==> Subsect_StrongNSCProblem.tex <==
%\section{Strongly $N$-Step Nonblocking Supervisory Control Problem}

We first introduce another new concept, called {\em heterogeneously quantitative nonblockingness}, which quantifies the nonblocking property of a generator by differentiating its marker states.


Let ${\bf G} = (Q,\Sigma,\delta,q_0,Q_m)$ be a generator (modeling the plant to be controlled) as in (\ref{eq:plant}) and assume that ${\bf G}$ is nonblocking.
Consider a specification $E \subseteq \Sigma^*$, and let ${\bf K} = (X,\Sigma,\xi,x_0,X_m)$ be a nonblocking generator
representing the language $E\cap L_m({\bf G})$, i.e. $L_m({\bf K}) = E \cap L_m({\bf G})$ and $\overline{L_m({\bf K})} = L({\bf K})$.
Define
\begin{align} \label{eq:QmK}
Q_m({\bf K}) := \{q_m \in Q_m| (\exists s\in \Sigma^*)~ &\xi(x_0, s) \in X_m \notag\\
~\& ~&\delta(q_0, s) = q_m \}.
\end{align}
Hence $Q_m({\bf K}) \subseteq Q_m$ is the subset of marker states of the plant $\bf G$ which corresponds to the imposed specification.
Note in general that not all marker states of the plant may be relevant to an imposed specification, and for the
control purpose of fulfilling the imposed specification $\bf K$, it suffices to consider those relevant marker states of $\bf G$ in $Q_m({\bf K})$. To rule out the trivial case, we assume that $Q_m({\bf K}) \neq \emptyset$.

Write $Q_m({\bf K}) = \{q_{m,i} | i \in \mathcal{I}\}$ ($\mathcal{I}$ is an index set).
For each $q_{m,i} \in Q_m({\bf K})$, define
\begin{align*} %\label{eq:str}
Rch_{\bf K}(q_{m,i}) := \{&x_m \in X_m|(\exists s \in \Sigma^*) \notag\\ &\xi(x_0, s) = x_m \& \delta(q_0,s) = q_{m,i}\};
\end{align*}
thus $Rch_{\bf K}(q_{m,i})$ includes all the marker states in $\bf K$ representing the same marked behavior as $q_{m,i}$ in $\bf G$.
Note that $Rch_{\bf K}(q_{m,i})$ is nonempty because $q_{m,i} \in  Q_m({\bf K})$.
Let $x \in X \setminus Rch_{\bf K}(q_{m,i})$ be an arbitrary state in $X$. We define the set of strings that lead $x$ to $Rch_{\bf K}(q_{m,i})$  for the first time, namely
\begin{align*} %\label{eq:SC}
C_{\bf K}(x,q_{m,i}):=\{s \in \Sigma^*| \xi(x,s)! ~\&~\xi(x,s) \in Rch_{\bf K}(q_{m,i})~\&\notag\\
     (\forall s' \in \overline{s}\setminus\{s\}) \xi(x,s') \notin Rch_{\bf K}(q_{m,i})\}
\end{align*}
If $x \in Rch_{\bf K}(q_{m,i})$, we define $C_{\bf K}(x, q_{m,i}) := \{\epsilon\}$.

Let $x \in X$ be an arbitrary state in $\bf K$, $q_{m,i} \in  Q_m({\bf K})$ an arbitrary marker state in $\bf G$, and $N_i$ a finite positive integer (which is
$q_{m,i}$ specific). We say that state $x$ is {\em $N_i$-step coreachable} (wrt. $q_{m,i}$) if
\begin{align*}
{\rm (i)} ~~ & C_{\bf K}(x, q_{m,i}) \neq \emptyset; \mbox{ and}\\
{\rm (ii)} ~~& (\forall s \in C_{\bf K}(x, q_{m,i})) ~|s| \leq N_i.
\end{align*}
Condition (i) ensures that for each marker state $q_{m,i} \in  Q_m({\bf K})$, there exists at least a string $s \in \Sigma^*$ leading $x$ to a marker state in $Rch_{\bf K}(q_{m,i})$. Note that by string $s$, the plant $\bf G$ will visit marker state $q_{m,i}$.
Condition (ii) means that all strings that lead $x$ to $Rch_{\bf K}(q_{m,i})$ for the first time have length at most $N_i$.
Intuitively, condition~(ii) means that in the worst case, it takes $N_i$ steps from state $x$ to complete the task represented by $q_{m,i}$.
Now we introduce the new concept of heterogeneously quantitative nonblockingness of a generator.

\smallskip
\begin{defn} \label{defn:snnbg}
Let ${\bf G}$ be a nonblocking generator, $\bf K$ be a nonblocking generator with $L_m({\bf K}) \subseteq L_m({\bf G})$, $Q_m({\bf K}) \subseteq Q_m$
a subset of marker states as defined in (\ref{eq:QmK}), and $N_i$ a positive integer for each $q_{m,i} \in Q_m({\bf K})$.
We say that ${\bf K}$ is \emph{heterogeneously quantitatively nonblocking} wrt. $\{(q_{m,i}, N_i)|i \in \mathcal{I}\}$ if for every marker state $q_{m,i} \in Q_m({\bf K})$
and every state $x \in X$, $x$ is $N_i$-step coreachable (wrt. $q_{m,i}$).
\end{defn}
\smallskip

This definition distinguishes each individual marker state (in $Q_m({\bf K})$), which is
in contrast with Definition~1 of quantitatively nonblocking generator
where all marker states are treated the same.

%In the above definition, every marker state $q_{m_i}$ (relevant to the specification) must be
%visited in $N_i$ steps; this requirement coincides with requirement (R2) that each marker state $q_{m,i}$ must be visited in bounded number of steps.

Next we define the heterogeneously quantitatively nonblocking property of a supervisory control $V$. For this, we first introduce a new concept called {\em heterogeneously quantitative completability}.

%For this, we first present a new concept called {\em heterogeneous quantitative language completability}.

%Consider the marked behavior $L_m({\bf G})$ of a nonblocking generator ${\bf G}$. Let
%$T := \{q_{m,i}\in Q_m | i\in \mathcal{I}\}$ ($\mathcal{I}$ is an index set) be a subset of marker states which must be visited in bounded number of steps, and $\mathcal{N} := \{N_i | i \in \mathcal{I}\}$ a set of positive integers, each $N_i$ corresponding
%to a $q_{m,i}$. We also use
%\begin{align} \label{eq:TN}
%(T, \mathcal{N}) = \{(q_{m,i}, N_i)| i\in \mathcal{I}\}
%\end{align}
%to denote the definitions of $T$ and $\mathcal{N}$, and their one to one relationship.

Let $K \subseteq L_m({\bf G})$ be a sublanguage of $L_m({\bf G})$, and define
\begin{align} \label{eq:QmKL}
Q_m(K) := \{q_m \in Q_m| (\exists s \in K)~ \delta(q_0, s) = q_m \}.
\end{align}
If $K$ is represented by a nonblocking generator $\bf K$, i.e. $L_m({\bf K}) = K$, then we have $Q_m(K) = Q_m({\bf K})$.
We also write $Q_m(K) = \{q_{m,i} | i \in \mathcal{I}\}$ ($\mathcal{I}$ is an index set).
For each $q_{m,i} \in Q_m(K)$, define
\begin{align} \label{eq:str}
Str_K(q_{m,i}):= \{s \in K | \delta(q_0,s) = q_{m,i}\};
\end{align}
then $Str_K(q_{m,i})$ includes all the strings in $K$ whose occurrences mean the completion of a marked behavior as represented by $q_{m,i}$.
Note that $Str_K(q_{m,i})$ is nonempty because $q_{m,i} \in Q_m(K)$.
For an arbitrary string $s \in \overline{K}$ and an arbitrary marker state $q_{m,i} \in Q_m(K)$, define the set of strings that lead $s$ to $Str_K(q_{m,i})$ for the first time:
\begin{align} \label{eq:PKL}
M_K(s,q_{m,i}):=\{&t \in \Sigma^* \mid st \in Str_K(q_{m,i}) \& \notag\\
&(\forall t' \in \overline{t} \setminus\{t\}) st' \notin Str_K(q_{m,i}) \}.
\end{align}
If $s \in Str_K(q_{m,i})$, we define $M_K(s, q_{m,i}) :=\{\epsilon\}$.

\smallskip
\begin{defn} \label{defn:sncomp}
Let ${\bf G}$ be a nonblocking generator, $K  \subseteq L_m({\bf G})$ a sublanguage, $Q_m(K) \subseteq Q_m$
a subset of marker states as defined in (\ref{eq:QmKL}), and $N_i$ a positive integer for each $q_{m,i} \in Q_m(K)$.
We say that $K$ is \emph{heterogeneously quantitatively completable} wrt. $\{(q_{m,i}, N_i)|i \in \mathcal{I}\}$ if
for all $s \in \overline{K}$ and all $q_{m,i} \in Q_m(K)$,
\begin{align*}
{\rm (i)}&~ M_K(s, q_{m,i}) \neq \emptyset;\\
{\rm (ii)}&~ (\forall t \in M_K(s, q_{m,i}))~ |t| \leq N_i.
\end{align*}
\end{defn}
\smallskip
%Note that distinguished with Definition~\ref{defn:ncomp} for quantitative completablility, the above definition
%additionally require condition (i); this condition guarantees
%that starting any string $s \in \overline{K}$, every marker state will be visited at least one time.
If $K$ is heterogeneously quantitatively completable, then for every marker state $q_{m,i} \in Q_m({K})$, every
string $s \in \overline{K} $ may be extended to a string in $Str_K(q_{m,i})$ (generating the marked behavior
represented by $q_{m,i}$) by strings of lengths at most $N_i$. Comparing with Definition~\ref{defn:ncomp} of quantitative completability, the above
definition distinguishes individual marker states (in $Q_m(K)$).

We illustrate Definition~\ref{defn:sncomp} by the following example, with emphasis on the difference from quantitative completability.
%\setlength{\floatsep}{5pt plus 2pt minus 2pt}
\begin{figure}[!t]
\centering
    \includegraphics[scale = 0.34]{Figures/K3prim.pdf}
\caption{Transition graph of ${\bf K}_3'$ } \label{fig:K3'}
\vspace{-0.2cm}
\end{figure}


\smallskip
\begin{example} [Continuing Example 1]
Reconsider the generator ${\bf G}$ in Example 1, and let $K_1, K_2, K_3 \subseteq  L_m({\bf G})$ be sublanguages
as represented by generators ${\bf K}_1$, ${\bf K}_2$ and ${\bf K}_3$ respectively (displayed in Fig.~\ref{fig:K123}).
For all these three cases $Q_m(K_i) = \{1, 2\}$.

First, although $K_1$ is quantitatively completable wrt. $N = 1$, it is not heterogeneously
quantitatively completable wrt. $\{(1, N_1 = 1),(2, N_2 = 1)\}$. This is because if the vehicle is at state 3, it is not guaranteed to arrive marker state 1 (corresponding to $Str_{K_1}(1)$) in one step.

Second, $K_2$ is not quantitatively completable wrt. any finite positive integer $N$, and by the same reason as described in Example 1 (the finite but unboundedly occurrences of string $19.17$) it is also not heterogeneously quantitatively completable wrt. any $\{(1, N_1),(2, N_2)\}$.

Third, $K_3$ is quantitatively completable wrt. $N = 4$, but it is not heterogeneously quantitatively completable wrt. $\{(1, N_1 = 4), (2, N_2 = 4)\}$, because
marker state 1 is not guaranteed to be arrived from state 2 in 4 steps. Also, $K_3$ is not heterogeneously quantitatively completable wrt. $\{(1, N_1 = 5), (2,N_2)\}$ for any positive integer $N_2$, because although marker state 1 can be arrived from any other state in 5 steps, but marker state 2  is not guaranteed to be arrived
from any other state in $N_2$ steps (due to the existence of string $(11.29)^{N_2}$).

Finally, remove transitions (1,21,4) and (1,12,0) from ${\bf K}_3$ and
denote the new generator by $K_3'$ (see Fig.~\ref{fig:K3'}). Let
$K_3' = L_m({\bf K}_3')$, and it is verified that $K_3'$ is both quantitatively completable wrt. $N = 5$ and heterogeneously quantitatively completable
wrt. $\{(1, N_1 = 5),(2, N_2 = 5)\}$. \hfill $\diamond$
\end{example}
\smallskip

%{\color{red}
%In Definition~\ref{defn:sncomp}, we need to identify the strings of $K$ that visits the same marker state; this definition coincides with
%requirement (R2) that the finite-step reachability of each marker states must be considered. According to Definitions~\ref{defn:ncomp} and \ref{defn:sncomp}, heterogeneous quantitative completability and quantitative completability cannot imply to each other.
%Only in the special case when the plant has exactly one marker state (i.e. $|Q_m| = 1$), $T = Q_m$ and $\mathcal{N} = \{N\}$,
%these two properties are the same.}
%\begin{pro} \label{pro:relation}
%Let ${\bf G}$ be a nonblocking generator, $N$ a finite positive integer, and $K \subseteq L_m({\bf G})$ a sublanguage.
%If $|Q_m| = 1$ (namely, $Q_m$ has only one marker state), then $K$ is strongly $N$-step completable wrt. $\bf G$ iff it is $N$-step completable.
%\end{pro}
%This result can be obtained immediately from Definitions~\ref{defn:ncomp} and %\ref{defn:sncomp}.

Note in general that Definitions~\ref{defn:ncomp} and \ref{defn:sncomp} do not
imply each other when there is no particular relationship between $N$ and $\{N_i| i \in \mathcal{I}\}$. But there are two special cases:
(i) when $|Q_m(K)| = 1$ and $N_i = N$, the two concepts are identical; (ii) when $N$ is greater than or equal to the minimum $N_i$,
if a language is heterogeneously quantitatively completable wrt. $\{(q_{m,i}, N_i)|i \in \mathcal{I}\}$, then it is quantitatively completable wrt. $N$. The first result is obvious, and the reason
for (ii) is as follows. Let $q_{m,i} \in Q_m(K)$ be the marker state corresponding to the minimum $N_i$. Required by heterogeneously quantitative completability,
every string $s \in \overline{K} $ may be extended to a string in $Str_K(q_{m,i})$ by strings of lengths at most $N_i$,
and thus $s$ can be extended to a string in $K$ (due to $Str_K(q_{m,i}) \subseteq K$). Thus $K$ is quantitatively completable wrt. the minimum $N_i$, and is in turn quantitatively completable wrt.
any other integer $N$ greater than or equal to the minimum $N_i$.


With the above newly introduced heterogeneously quantitative  language completability, we introduce a heterogeneously quantitatively nonblocking property of a supervisory control.

\smallskip
\begin{defn} \label{defn:snnbs}
Let ${\bf G}$ be a nonblocking generator, $K  \subseteq L_m({\bf G})$ a sublanguage, $Q_m(K) \subseteq Q_m$
a subset of marker states as defined in (\ref{eq:QmKL}), $N_i$ a positive integer for each $q_{m,i} \in Q_m(K)$,
and $V : L({\bf G}) \rightarrow \Gamma$ a (marking) supervisory control (for $(K,{\bf G})$).
We say that $V$ is \emph{heterogeneously quantitatively nonblocking} wrt. $\{(q_{m,i}, N_i)|i \in \mathcal{I}\}$ if
\vspace{-0.2cm}
\begin{align*}
{\rm (i)} ~~ &V \text{ is nonblocking}; \mbox{ and}\\
{\rm (ii)} ~~& L_m(V/{\bf G})~\text{is heterogeneously quantitatively } \\
&\text{completable wrt. $\{(q_{m,i}, N_i)|i \in \mathcal{I}\}$.}
\end{align*}
\end{defn}
\smallskip

According to Definitions~\ref{defn:snnbg} and \ref{defn:sncomp},
a language $K$ is heterogeneously quantitatively completable wrt. $\{(q_{m,i}, N_i)|i \in \mathcal{I}\}$ iff the generator $\bf K$ representing $K$ is heterogeneously quantitatively nonblocking wrt. $\{(q_{m,i}, N_i)|i \in \mathcal{I}\}$.
Thus when the closed-loop system $V/{\bf G}$ is represented by a (nonblocking) generator $\bf CG$ (say), i.e. $L_m({\bf CG}) = L_m(V/{\bf G})$ and
$L({\bf CG}) = L(V/{\bf G})$, if $V$ is heterogeneously quantitatively nonblocking wrt. $\{(q_{m,i}, N_i)|i \in \mathcal{I}\}$, then the generator $\bf CG$
is heterogeneously quantitatively nonblocking wrt. $\{(q_{m,i}, N_i)|i \in \mathcal{I}\}$. Namely, the closed-loop system $V/{\bf G}$ has the property of heterogeneously quantitative nonblockingness,
and thus satisfies the requirement (R2).

%Condition~(i) means that $\overline{L_m(V/{\bf G})} = L(V/{\bf G})$, while
%condition~(ii) means that $L_m(V/{\bf G})$ is strongly $N$-step completable wrt. $Q_m^N$.

We are ready to formulate the \emph{Heterogeneously Quantitatively Nonblocking Supervisory Control Problem} of DES ({\em HQNSCP}).

{\it Consider a DES plant modeled by a generator ${\bf G} = (Q,\Sigma_c \dot\cup \Sigma_{uc},\delta,q_0,Q_m)$, a specification language $E \subseteq \Sigma^*$, and let  $K := E\cap L_m({\bf G})$,
$Q_m(K)$ as defined in ~(\ref{eq:QmKL}), and $N_i$ a positive integer for each $q_{m,i} \in Q_m(K)$.
Construct a (marking) supervisory control $V: L({\bf G})\rightarrow \Gamma$ %(for $(K, {\bf G})$)
satisfying the following properties:
\begin{itemize}
\item[$\bullet$]  {\bf Safety}. Marked behavior of the closed-loop system $V/{\bf G}$ satisfies the imposed specification $E$ in the sense that {$L_m(V/{\bf G}) \subseteq E\cap L_m({\bf G})$}.%$L_m(V/{\bf G}) = K \subseteq E\cap L_m({\bf G}) = K$.

\item[$\bullet$] {\bf Heterogeneously quantitative nonblockingness}. Supervisory control $V$ is heterogeneously quantitatively nonblocking wrt. $\{(q_{m,i}, N_i)|i \in \mathcal{I}\}$.

\item[$\bullet$] {\bf Maximal permissiveness}. Supervisory control $V$ does not restrict more behavior than necessary to satisfy
safety and heterogeneously  quantitative nonblockingness, i.e. for all
other supervisory controls $V'$ it holds that  $L_m(V'/{\bf G}) \subseteq L_m(V/{\bf G})$.
\end{itemize}
}

The above HQNSCP is also a generalization of the traditional nonblocking supervisory control problem \cite{RamWon87,WonRam87,Wonham16a}, in that the second requirement of heterogeneously quantitative nonblockingness is stronger than the traditional nonblockingness. This generalized problem cannot be solved in general by supervisors synthesized using the standard method. Also note that HQNSCP cannot be solved by the method introduced above for solving QNSCP. For example, with the same $\bf G$, $E$ and $N = 3$, the supervisor
$\bf QSUP$ in Fig. ~\ref{fig:NCSUP} cannot solve HQNSCP wrt. $\{(1,N_1 = N),(2, N_2 = N)\}$, because if the vehicle is in zone~3 (state 3), it is not guaranteed to arrive zone 1 (state 1) in three steps.
In the rest of this section we will present a solution for HQNSCP.

\begin{remark}
We note in \cite{QueirozEt:2005} that multitasking supervisory control of DES considers a requirement
where there are multiple tasks and each task must be completed. This requirement is  expressed as strong nonblockingness of automaton. However, the bound on the number of steps completing each task is not considered, and consequently the developed method in \cite{QueirozEt:2005} cannot be
applied to solve our problem HQNSCP.

%In heterogeneously quantitatively nonblockingness, we distinguish each marker state of the plant as a task, while
%in  \cite{QueirozEt:2005} a task may be represented by a subset of states; namely in our paper
%\[C = \{c_i ~| ~\text{each}~ c_i~ \text{corresponds to a marker state }~ q_{m_i \in Q_m}\}.\] In this case, there
%exists the maximally permissive supervisor satisfying (quantitative) nonblockingness. However, we presented in \cite{ZhangWangCaiArxiv:2021}
%a example which shows that there may not exist the maximally permissive supervisor by multitasking supervisory control in \cite{QueirozEt:2005}.


%According to the definition of marking function $\chi:Q\rightarrow Pwr(C)$ in the definition of colored marking generator,
%one state $q \in Q$ may be assigned with different colors e.g. $c_1$ and $c_2$.
%If there is no bound on the number of steps imposed on each color, it is proved in \cite{QueirozEt:2005} that there exists maximally permissive
%supervisor satisfying strongly nonblockingness. Considering the bound on completing each task, we assign one color with a bound to represent that a
%task represented by the color must be completed in a bounded number of transition steps.
%In that case, one state $q$ may be required to be visited in different number of steps, e.g. $N_1$ for $c_1$ and $N_2$ for $c_2$.
%Since the control policy on each state should be deterministic, the bound on $q$ should be unique.
%Assuming that $N_1 < N_2$, the bound on this state is naturally set to be the smaller $N_1$; otherwise, the requirement $N_1$
%for $c_1$ cannot be satisfied. However, by this rule, the following example as shown in Fig.~\ref{fig:remark} (assuming that $\chi(1) = c_1$, $\chi(2) = \{c_1, c_2\}$) demonstrates that the supervisor may not be maximally permissive for satisfying $N_1 = 2$ for $c_1$ and $N_2 = 3$ for $c_2$.
%
%\begin{figure}[!t]
%\centering
%    \includegraphics[scale = 0.35]{Figures/NKK1.pdf}
%\caption{Transition graphs of automata representing $K$ and $K_1$ in Remark 1} \label{fig:remark}
%\end{figure}
%
%Since $\chi(2) = \{c_1, c_2\}$, we may set $N_2 = 2$ on $c_2$. In this case, state 4 in ${\bf K}$ should be removed, because
%at state 0, the task $c_2$ is not guaranteed to be completed in two steps. Thus, we get ${\bf K}_1$ which is strongly nonblocking
%with respect to $N_1 = 2$ for $c_1$ and $N_2 = 2$ for $c_2$. However, it is easily verified that ${\bf K}$ is strongly nonblocking
%with respect to $N_1 = 2$ for $c_1$ and $N_2 = 3$ for $c_2$, which is more permissive than ${\bf K}_1$. In our paper, each marker
%state has a corresponding unique bound, and we have shown that there exists the maximally-permissive heterogeneous quantitative nonblocking supervisor.

%Hence, the work in \cite{QueirozEt:2005} cannot be directly applied to the case described in our paper, where each marker state represents a task and the task must be completed in bounded number of steps. We may investigate in future work that in which case, there exists the maximally permissive strongly nonblocking supervisor
%in MTDES (multitasking discrete-event systems) with the bounds required on completing tasks.
\end{remark}



